Segment and Caption Anything

We propose a method to efficiently equip the Segment Anything Model (SAM) with the ability to generate regional captions. SAM presents strong generalizability to segment anything while is short for semantic understanding. By introducing a lightweight query-based feature mixer, we align the region-specific features with the embedding space of language models for later caption generation. As the number of trainable parameters is small (typically in the order of tens of millions), it costs less computation, less memory usage, and less communication bandwidth, resulting in both fast and scalable training. To address the scarcity problem of regional caption data, we propose to first pre-train our model on objection detection and segmentation tasks. We call this step weak supervision pretraining since the pre-training data only contains category names instead of full-sentence descriptions. The weak supervision pretraining allows us to leverage many publicly available object detection and segmentation datasets. We conduct extensive experiments to demonstrate the superiority of our method and validate each design choice. This work serves as a stepping stone towards scaling up regional captioning data and sheds light on exploring efficient ways to augment SAM with regional semantics. The project page, along with the associated code, can be accessed via https://xk-huang.github.io/segment-caption-anything/.

==> tabs/comp-ref-vllm.tex <==

\begin{table}[t]
\centering
\caption{
Comparison with referring Vision Large Language Models (VLLMs).
``M'': Meteror, ``C'': CIDEr-D.
$\dagger$: The scores are from the papers. 
$\ddagger$: We reproduced the result with ``GPT4RoI-7B-delta-V0'' from \url{https://github.com/jshilong/GPT4RoI}. 
The best, the second best, the third best scores are marked as \colorbox[rgb]{1,0.698,0.698}{\strut red}, \colorbox[rgb]{1,0.851,0.698}{\strut orange}, \colorbox[rgb]{0.996,1,0.698}{\strut yellow}, respectively.
}
\label{supp:tab:comp-ref-vllm}
\begin{tabular}{lcc} 
\toprule
Method                        & {M}                  & {C}                    \\ 
\hline
ASM~\cite{wangAllSeeingProjectPanoptic2023} (Zero-shot)$^\dagger$                & 12.6                                 & 44.2                                   \\
ASM (Finetuned)$^\dagger$                & {\cellcolor[rgb]{1,0.698,0.698}}18.0 & 145.1                                  \\

GPT4RoI~\cite{zhangGPT4RoIInstructionTuning2023a} (7B)$^\dagger$                   & 17.4                                 & 145.2                                  \\
GPT4RoI (13B)$^\dagger$                 & {\cellcolor[rgb]{1,0.851,0.698}}17.6 & 146.8                                  \\
GPT4RoI (7B)$^\ddagger$                 & 16.4 & 122.3     \\
\hline
SCA (GPT2-large, VG)          & 17.4                                 & {\cellcolor[rgb]{0.996,1,0.698}}148.8  \\
SCA (LLAMA-3B, VG)            & 17.4                                 & {\cellcolor[rgb]{1,0.851,0.698}}149.8  \\
SCA (GPT2-large, Pretrain+VG) & {\cellcolor[rgb]{0.996,1,0.698}}17.5 & {\cellcolor[rgb]{1,0.698,0.698}}149.8  \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/data-stats.tex <==
\begin{table*}[t]
\centering
\caption{The statistics of region-level understanding datasets used for training. }
\label{tab:exp:data_stats}
\begin{tabular}{l|crrrrr}
\toprule
dataset                          & type        & total samples & total regions & total sents & total tokens & total words \\
\midrule
COCO\cite{linMicrosoftCOCOCommon2015a_mscoco}                   & Region recognition & 117,266       & 860,001       & 860,001     & 1,275,513    & 942,822     \\
V3Det~\cite{wangV3DetVastVocabulary2023a}                     & Region recognition & 183,348       & 1,357,351     & 1,357,351   & 3,984,388    & 2,126,318   \\
Objects365~\cite{shaoObjects365LargeScaleHighQuality2019}                & Region recognition & 1,742,289     & 25,407,598    & 25,407,598  & 49,264,696   & 32,341,116  \\
\midrule
Visual Genome~\cite{krishnaVisualGenomeConnecting2016a_VG} & Region captioning  & 77,398        & 3,684,063     & 3,684,063   & 21,392,494   & 19,740,221  \\
\color{gray} RefCOCOg~\cite{yuModelingContextReferring2016a_refcoco}                  & \color{gray} Referring Expression  & \color{gray} 24,698        & \color{gray} 48,599        & \color{gray} 92,671      & \color{gray} 834,305      & \color{gray} 785,259     \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/implem_details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The implementation details. $\ast$: As the batch size ramps up, the image epoch and region epochs are subjected to be changed, and the learning rate will be scaled linearly \wrt the batch size.}
\label{sec3:tab:implem_details}
{%
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{l}{Optimization}                              \\
\hline
\multirow{2}{*}{Optimizer}    & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}AdamW\\ (0.9, 0.999) \\ \hline \end{tabular}}                  \\
                        &                  \\
LR $^\ast$                      & 0.0001                              \\
LR Decay Ratio          & 0                                   \\
LR Decay                & cosine                              \\
Weight Decay            & 0.0001                              \\
Warmup ratio            & 0.3333                              \\
Warmup steps            & 200                                 \\
Gradient Clipping       & 1.0                                 \\
\toprule
\multicolumn{2}{l}{Data Epoch$^\ast$}                                \\
\hline
Batch Size$^\ast$              & 8                                   \\
\# Reg / Img            & 16                                  \\
Steps                   & 200000                              \\
\# Img                  & 77398                               \\
\# Reg                  & 3684063                             \\
Img Epoch$^\ast$               & 20.67                               \\
Reg Epoch$^\ast$               & 6.95                                \\
GPU Type                & V100-16GB                           \\
\# GPUs                 & 8                                   \\
\toprule
\multicolumn{2}{l}{Model Details}                           \\
\hline
\multirow{5}{*}{Input} & \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}} a) 1024x1024\\ Long side: 1024\\ Short side: padding \\b) Large Scale Jitter\\ c) Horizontal Flip \\ \hline \end{tabular}} \\
                        &                  \\
                        &                  \\
                        &                  \\
                        &                  \\
\multirow{2}{*}{Loss}         & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} a) Cross Entropy Loss\\ b) Label Smooth (0.1) \\ \hline \end{tabular}} \\
                        &                  \\
\multirow{2}{*}{Text Decoder} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} a) GPT2-large\\ b) Open LLAMA 3B v2 \\ \hline \end{tabular}}       \\
                        &                  \\
\# Query Tokens         & 8                                   \\
\# Mixer Layers         & 12                                  \\
\# Task Tokens          & 6                                   \\
Opt. Module             & Text Feat. Mixer                    \\
\# Opt. Params          & 19.4 M                              \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tabs/other_image_feature.tex <==
% \usepackage{colortbl}
% \usepackage{booktabs}


\begin{table}[th]
\centering
\caption{Comparison of using different image encoders. ``C'': CIDEr-D, ``M'': Meteror.}
\label{supp:tab:other_image_encoders}
\begin{tabular}{lcc} 
\toprule
Image
  Encoder                           & {C}             & {M}              \\ 
\hline
vit\_large\_patch14\_clip\_336.openai     & 67.3  & 10.2 \\
vit\_large\_patch14\_clip\_224.datacompxl & 59.0  & 9.3  \\
eva02\_large\_patch14\_clip\_336.merged2b & 53.9  & 8.8  \\
vit\_large\_patch14\_reg4\_dinov2.lvd142m & 76.4  & 11.2 \\
vit\_large\_patch16\_224.mae              & 59.6  & 9.4  \\
\hline
\textit{Add optimization of sam feature mixer}   &         &        \\
vit\_large\_patch14\_clip\_336.openai     & 66.7  & 10.1 \\
vit\_large\_patch14\_clip\_224.datacompxl & 60.3  & 9.5  \\
eva02\_large\_patch14\_clip\_336.merged2b & 54.2  & 8.8  \\
vit\_large\_patch14\_reg4\_dinov2.lvd142m & 76.1  & 11.1 \\
vit\_large\_patch16\_224.mae              & 59.2  & 9.4  \\
\hline
\textit{SAM}                                       & {}                    & {}                    \\
SAM-ViT-base                              & {\cellcolor[rgb]{1,0.851,0.698}}130.2 & {\cellcolor[rgb]{1,0.698,0.698}}16.0  \\
SAM-ViT-large                             & {\cellcolor[rgb]{0.996,1,0.698}}129.6 & {\cellcolor[rgb]{0.996,1,0.698}}15.9  \\
SAM-ViT-huge                              & {\cellcolor[rgb]{1,0.698,0.698}}130.9 & {\cellcolor[rgb]{1,0.851,0.698}}16.0  \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/zero-shot-reg.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}


\begin{table*}[t]
\centering

\caption{
The zero-shot performance on the Referring Expression Generation (REG) task. ``M'': Meteror, ``C'': CIDEr-D. 
$\ast$: ``k'' means the number of examples in the prompt.
$\dagger$: The scores are from the papers.
}
\label{supp:tab:zero-shot-reg}
\begin{tabular}{l|cc|cccc|cccc} 
\toprule
\multirow{3}{*}{Method}       & \multicolumn{2}{c|}{RefCOCOg}                                                                        & \multicolumn{4}{c|}{RefCOCO+}                                                                                                                                                                              & \multicolumn{4}{c}{RefCOCO}                                                                                                                                                                                 \\ 
\cline{2-11}
                              & \multicolumn{2}{c|}{val}                                                                             & \multicolumn{2}{c}{testA}                                                                           & \multicolumn{2}{c|}{testB}                                                                           & \multicolumn{2}{c}{testA}                                                                           & \multicolumn{2}{c}{testB}                                                                             \\ 
\cline{2-11}
                              & M             & C                                                    & M             & C                                                    & M             & C                                                    & M             & C                                                    & M             & C                                                      \\ 
\hline
\textit{separate train/test}                                & {}                   &                                                            &                                                            &                                                            &                                                            &                                                            &                                                            &                                                            &                                                              \\
Visdif~\cite{yuModelingContextReferring2016a_refcoco}$^\dagger$                        & 14.5                                 & {-}                  & {14.2}                                 & -                                                          & {13.5}                                 & -                                                          & {18.5}                                 & -                                                          & {{\cellcolor[rgb]{1,0.851,0.698}}24.7} & -                                                            \\
SLR~\cite{yuJointSpeakerListenerReinforcerModel2017a_slr_refcoco}$^\dagger$                           & {\cellcolor[rgb]{1,0.698,0.698}}15.9 & 66.2                                 & {21.3}                                 & {{\cellcolor[rgb]{1,0.698,0.698}}52.0} & {{\cellcolor[rgb]{1,0.698,0.698}}21.5} & {{\cellcolor[rgb]{1,0.698,0.698}}73.5} & {{\cellcolor[rgb]{1,0.698,0.698}}29.6} & {{\cellcolor[rgb]{1,0.698,0.698}}77.5} & {{\cellcolor[rgb]{1,0.698,0.698}}34.0} & {{\cellcolor[rgb]{1,0.698,0.698}}132.0}  \\ 
\hline
\textit{zero-shot}                     & {}                   & {}                   &                                                            &                                                            &                                                            &                                                            &                                                            &                                                            &                                                            &                                                              \\
Kosmos-2~\cite{pengKosmos2GroundingMultimodal2023a}$^\dagger$                      & 12.2                                 & 60.3                                 & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                            \\
Kosmos-2 (k=2)$^\ast$$^\dagger$                & 13.8                                 & 62.2                                 & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                            \\
Kosmos-2 (k=4)$^\ast$$^\dagger$                 & 14.1                                 & 62.2                                 & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                            \\
ASM~\cite{wangAllSeeingProjectPanoptic2023}$^\dagger$                           & 13.6                                 & 41.9                                 & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                            \\
GRiT~\cite{wuGRiTGenerativeRegiontotext2022a}                          & 15.2                                 & {\cellcolor[rgb]{0.996,1,0.698}}71.6 & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                          & -                                                            \\
SCA (GPT2-large, Pretrain+VG) & {\cellcolor[rgb]{0.996,1,0.698}}15.4 & {\cellcolor[rgb]{1,0.851,0.698}}71.9 & {{\cellcolor[rgb]{0.996,1,0.698}}21.7} & {29.2}                                 & {{\cellcolor[rgb]{1,0.851,0.698}}20.4} & {{\cellcolor[rgb]{1,0.851,0.698}}57.2} & {20.4}                                 & {27.0}                                 & {20.2}                                 & {{\cellcolor[rgb]{0.996,1,0.698}}66.4}   \\
SCA (GPT2-large, VG)          & 15.3                                 & 70.5                                 & {{\cellcolor[rgb]{1,0.851,0.698}}21.7} & {{\cellcolor[rgb]{1,0.851,0.698}}30.2} & {20.1}                                 & {{\cellcolor[rgb]{0.996,1,0.698}}56.6} & {{\cellcolor[rgb]{0.996,1,0.698}}20.5} & {{\cellcolor[rgb]{1,0.851,0.698}}27.7} & {20.1}                                 & {{\cellcolor[rgb]{1,0.851,0.698}}66.7}   \\
SCA (LLAMA-3B, VG)            & {\cellcolor[rgb]{1,0.851,0.698}}15.6 & {\cellcolor[rgb]{1,0.698,0.698}}74.0 & {{\cellcolor[rgb]{1,0.698,0.698}}22.0} & {{\cellcolor[rgb]{0.996,1,0.698}}30.0} & {{\cellcolor[rgb]{0.996,1,0.698}}20.2} & {56.1}                                 & {{\cellcolor[rgb]{1,0.851,0.698}}20.7} & {{\cellcolor[rgb]{0.996,1,0.698}}27.3} & {{\cellcolor[rgb]{0.996,1,0.698}}20.3} & {65.3}                       \\
\bottomrule
\end{tabular}
\end{table*}
